Simple Circuit Extensions for XOR in PTIME

The Minimum Circuit Size Problem for Partial Functions ($MCSP^*$) is hard assuming the Exponential Time Hypothesis (ETH) (Ilango, 2020). This breakthrough hardness result leveraged a characterization of the optimal $\{\land, \lor, \neg\}$ circuits for $n$-bit $OR$ ($OR_n$) and a reduction from the partial $f$-Simple Extension Problem where $f = OR_n$. It remains open to extend that reduction to show ETH-hardness of total $MCSP$. However, Ilango observed that the total $f$-Simple Extension Problem is easy whenever $f$ is computed by read-once formulas (like $OR_n$). Therefore, extending Ilango's proof to total $MCSP$ would require one to replace $OR_n$ with a slightly more complex but similarly well-understood Boolean function. This work shows that the $f$-Simple Extension problem remains easy when $f$ is the next natural candidate: $XOR_n$. We first develop a fixed-parameter tractable algorithm for the $f$-Simple Extension Problem that is efficient whenever the optimal circuits for $f$ are (1) linear in size, (2) polynomially "few" and efficiently enumerable in the truth-table size (up to isomorphism and permutation of inputs), and (3) all have constant bounded fan-out. $XOR_n$ satisfies all three of these conditions. When $\neg$ gates count towards circuit size, optimal $XOR_n$ circuits are binary trees of $n-1$ subcircuits computing $(\neg)XOR_2$ (Kombarov, 2011). We extend this characterization when $\neg$ gates do not contribute the circuit size. Thus, the $XOR$-Simple Extension Problem is in polynomial time under both measures of circuit complexity.

==> figures/tikz/cone.tex <==
\usetikzlibrary{shapes.geometric}

\makeatletter
\pgfdeclareshape{cone}{
  \inheritsavedanchors[from=isosceles triangle] 
  \inheritanchor[from=isosceles triangle]{center}
  \inheritanchor[from=isosceles triangle]{apex}
  \inheritanchor[from=isosceles triangle]{left corner}
  \inheritanchor[from=isosceles triangle]{right corner}

\backgroundpath{
    % Store coordinates immediately in your own variables
    \pgf@anchor@cone@center
    \edef\centerx{\the\pgf@x}
    \edef\centery{\the\pgf@y}
    
    \csname pgf@anchor@cone@left corner\endcsname
    \edef\leftx{\the\pgf@x}
    \edef\lefty{\the\pgf@y}
    \pgfmathsetmacro{\radius}{sqrt(\leftx*\leftx + \lefty*\lefty)/4.5}
    %\pgftext[at={\csname pgf@anchor@cone@left corner\endcsname}, left]{\radius}
    
    \csname pgf@anchor@cone@right corner\endcsname  
    \edef\rightx{\the\pgf@x}
    \edef\righty{\the\pgf@y}

    \csname pgf@anchor@cone@apex\endcsname  
    \edef\apexx{\the\pgf@x}
    \edef\apexy{\the\pgf@y}
 
    % Calculate control point using stored values
    \pgfmathsetmacro{\controlx}{2*\leftx}
    \pgfmathsetmacro{\controly}{\centery}
    
    % Draw your path...
    \pgfsetcornersarced{\pgfpoint{\radius}{\radius}}
    \pgfpathmoveto{\pgf@anchor@cone@apex}
    \pgfpathlineto{\pgfpoint{\leftx}{\lefty}}
    \pgfpathquadraticcurveto{\pgfpoint{\controlx pt}{\controly pt}}{\pgfpoint{\rightx}{\righty}}
    \pgfpathlineto{\pgf@anchor@cone@apex}
}
}
\makeatother


==> figures/tikz/xor-proof/xor-proof-tikz-settings.tex <==
    \tikzset{node/.style={circle, draw, minimum size=0.75cm}}
    \tikzset{mnode/.style={circle, draw, dashed,minimum size=0.75cm}}
    \tikzset{output/.style={circle, node contents = {}}}
    \tikzset{padding/.style={circle, node contents = {}}}
    \tikzset{e/.style={thick}}
    \tikzset{w/.style={thick, dashed}}
    \tikzset{node distance = 0.75cm}
    \tikzset{>=latex}
